FFT Convolutions are Faster than Winograd on Modern CPUs, Here is Why

Winograd-based convolution has quickly gained traction as a preferred approach to implement convolutional neural networks (ConvNet) on various hardware platforms because it requires fewer floating point operations than FFT-based or direct convolutions. This paper compares three highly optimized implementations (regular FFT--, Gauss--FFT--, and Winograd--based convolutions) on modern multi-- and many--core CPUs. Although all three implementations employed the same optimizations for modern CPUs, our experimental results with two popular ConvNets (VGG and AlexNet) show that the FFT--based implementations generally outperform the Winograd--based approach, contrary to the popular belief. To understand the results, we use a Roofline performance model to analyze the three implementations in detail, by looking at each of their computation phases and by considering not only the number of floating point operations, but also the memory bandwidth and the cache sizes. The performance analysis explains why, and under what conditions, the FFT--based implementations outperform the Winograd--based one, on modern CPUs.

==> Makefile <==
DOC = $(notdir $(shell pwd))
DOC=main

# This line is intentionally blank.

OTHERS = Makefile

DEPS_DIR = .deps

LATEXMK=latexmk -pdf -dvi- -ps- -recorder -deps \
                  -pdflatex='pdflatex --shell-escape %O %S' \
                  -e 'show_cus_dep();' \
                  # -e 'warn qq(In Makefile, turn off custom dependencies);' \


default: pdf
.PHONY:  pdf default all remake clean test

test:
	echo $(DOC)

$(DEPS_DIR) :
	mkdir $@


%.w18:
	touch $@

###########################################################################
## Make targets for cleaning

clean:
	rm -f $(DOC).pdf $(DOC).aux $(DOC).log $(DOC).out $(DOC).brf $(DOC).code $(DOC).code.out $(DOC).fdb_latexmk $(DOC).fls $(DOC).bbl $(DOC).blg .deps/$(DOC).pdfP *~ $(DOC).dvi $(DOC).w18


###########################################################################
## Make targets for document

pdf : $(DOC).pdf

-include $(DEPS_DIR)/$(DOC).pdfP

%.w18 :
	touch $@

%.pdf : %.tex $(OTHERS)
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	$(LATEXMK) -deps-out=$(DEPS_DIR)/$@P $<
	if [ -e $@ ]; then touch $@; fi

remake :
	if [ ! -e $(DEPS_DIR) ]; then mkdir $(DEPS_DIR); fi
	$(LATEXMK) -g -deps-out=$(DEPS_DIR)/$(DOC).pdfP $(DOC).tex
	if [ -e $(DOC).pdf ]; then touch $(DOC).pdf; fi


==> section/estimates.tex <==
\subsection{Performance Comparison}

  For a given layer, when using the Winograd or FFT methods, the total
  number of operations, \DM, \AI~and thus the running time, will depend on
  the choice of $m$ ($r$ is determined by the layer's kernel sizes).

  \paragraph{Maximal Allowed Tile Sizes}

  Generally, larger values of $m$ decrease both the number of required
  operations and the amount of data movements (\DM) in all the
  methods, and thus, are more efficient.  However, in some cases, when
  the images need a substantial amount of zero--padding, a larger $m$
  can yield an increase in both the number of operations and data
  movements~\cite{winograd, lavin2016fast}.

  The numerical inaccuracy of Winograd convolutions increases
  exponentially with tile sizes, and thus with $m$~\cite{pan2016bad,
    winograd, lavin2016fast}.  In practice, there is an upper bound on
  the tile size for which the Winograd produces accurate enough
  results.  All major vendors, such as FALCON, MKL-DNN, LIBXSMM,
  and cuDNN~\cite{falconlib,libxsmmGit,mkl-dnn,cudnn} implement the
  Winograd algorithm with tile sizes less than or equal to $6\times 6$,
  which produces results with accuracy comparable to the one of direct
  convolution~\footnote{Applying the formula for convolution
    directly}.  For the performance comparison in this paper, we
  follow this convention, and consider only Winograd algorithms with
  tile sizes of at most $6 \times 6$.  In the appendix, we repeat some
  of the analysis and experiments with tile sizes up to $8 \times 8$
  as some recent research~\cite{vincent2017improving} has demonstrated
  that lower accuracy convolutions, in particular cases, can produce
  similar results.

  In contrast, the FFT methods have extremely high accuracy,
  higher than direct convolution, even for very large tile sizes (very
  large $m$).  Thus, we allow for an arbitrary tile sizes.  We analyze
  the impact of tile sizes to numerical accuracy of all the methods in
  detail in Sec.~\ref{sub_sec_accuracy}.

  The accuracy of the numerical computation for each individual layer
  should not be confused with the prediction accuracy of a ConvNet.
  Higher numerical accuracy does not imply faster training or better
  predictions.  However, a certain level of numerical accuracy is
  necessary (and sufficient)~\cite{courbariaux2014low, gupta2015deep}
  for ConvNet stability, above which the ConvNets are expected to
  perform the same.

  When comparing two methods, we compare the running times of each method
  using $m$ for which the running time is minimized:

  \begin{equation}
    \small
    \begin{aligned}
      Speedup^{\FFTs} &= \frac{\underset{m_W}{\min}\big \{Runing~time^{\WINs(m_W^2,r^2)}\big \}}
      {\underset{m_F}{\min}\big \{Running~time^{\FFTs(m_F^2,r^2)} \big \}}
    \end{aligned}\label{eq_new_speedup}
  \end{equation}

  where $m_W$ is the $m$ used for the Winograd method, and $m_F$ used
  for the Regular--FFT.  Similar equation can be derived for the
  Gauss--FFT method.

  \subsection{Theoretical Predictions}

  We explore the impact of various parameters of convolutional layers
  to the relative performances of the three methods.

  We start from a sample layer, the VGG layer 3.2, which has the batch
  size $B = 64$, 256 input and output channels ($C = C' = 256$).  The
  input image sizes are $58 \times 58$, and kernel sizes are $3 \times
  3$.  This can be considered an average layer.  Earlier layers in VGG
  have larger images, but less channels, whereas the latter layers
  have smaller images and more channels.  To understand the effect of
  each layer parameter, as well as cache size and \CMR~to the relative
  performances of FFT methods and Winograd method, we vary each of the
  parameters and show the estimated speedup of the FFT methods over
  Winograd, as well as Regular--FFT over Gauss--FFT.

  \begin{figure*}[ht]
    \begin{center}
      \includegraphics[width=0.95\linewidth]{__fig/vary_params.pdf}\\
    \end{center}
    \caption{Predictions of our model on the VGG layer 3.2, with various layer parameters, as well as the cache size varied.}
    \label{fig:model-predictions}
  \end{figure*}

  Fig.~\ref{fig:model-predictions} shows the model's predictions when
  different parameters of the layer or system are varied.  We assume
  $256$ KB of cache per core is available, except for the plot where
  the cache size is varied.

  Generally, the expected speedup of Regular--FFT over both Winograd
  and Gauss--FFT increases as the system's \CMR~ increases, whereas
  the relative speedup of Gauss--FFT over Winograd decreases.
  However, in certain cases, where the image sizes are relatively
  small, for a range of \CMR~, the relative speedup of Regular--FFT
  over Winograd first decreases until a certain \CMR, after which it
  starts to increase.

  To give some basic rules of thumb for how different parameters
  affect the relative performances of the three methods, we examine
  the differences of the differently colored lines.  When comparing
  the Regular--FFT and Winograd, when the L2 cache is varied (top left
  plot on Fig.~\ref{fig:model-predictions}), the red line,
  representing the mode predictions on systems with $64 KB$ cache is
  above the line representing systems with $128 KB$ cache, etc.  Thus,
  the relative performances of Regular--FFT method vs the Winograd
  method increase as the available cache size decreases.  Same
  conclusion can be made for varying layer's image sizes.

  When either the {\bf cache size} or {\bf input/output channels}
  decrease, the relative performances of both FFT methods over
  Winograd, as well as the relative performances of Regular--FFT over
  Gauss--FFT, increase.  The relative performances of both FFT methods
  over the Winograd method increase as either the {\bf kernel sizes},
  or the {\bf image sizes}, increase.  However, the kernel and the
  image sizes have no effect on the relative performances between the
  two FFT methods.


==> section/orig_bounds.tex <==
%\subsection{origin section 4}
 %
  %Besides the estimated FLOPs for each stage, we beet to estimate the
  %amount of main memory that has to be accessed (either read from, or
  %stored to) by each stage.  On a processor capable of $S_C$ FLOPS,
  %with a memory throughput $S_M$ bytes/s, the time required for
  %performing all arithmetic computation is at least $N_C/S_C$ and the
  %time required for all memory accesses is at least $N_M/S_M$.  Here,
  %$N_C$ is the number of FLOPs required by the stage, and $N_M$ is the
  %amount of memory that has to be accessed.  Modern processors are
  %capable of performing arithmetic computation and memory accesses at
  %the same time, thus, the bound on the time required for a given
  %stage is $\max\{N_C/S_C,N_M/S_M\}$.
	%
  %When $N_C/S_C$ is greater than $N_M/S_M$ we say that the stage is
  %compute bound -- the time required for performing the stage's
  %computation is bound by the peak FLOPS of the given processor.
  %Otherwise, we say that the stage is memory bound -- bound by the
  %memory throughput of the processor.
%
  %The compute--to--memory ratio of a given processor is defined as
  %$S_R = S_C/S_M$.  Similarly, the compute--to--memory ratio of a an
  %algorithm is defined by $N_R = N_C/N_M$.  We can rewrite the
  %equation above as: {\small
    %\label{eqn:times}
  %\begin{equation}
    %\frac{N_M}{S_C}\min\{N_R,S_R\}
  %\end{equation}
  %} Thus, whether a given stage is compute or memory bound depends on
  %the compute--to--memory ratio of the processor and the stage's
  %computation, and not the absolute values of the processors peak
  %FLOPS performances or memory throughput.
%
  %In the rest of the section, we show how to, for a given layer,
  %estimate the lower bound on the computation time, on a given
  %processor, for each stage of a Winograd/FFT/FFT+Gauss convolution
  %algorithms, as a function of $S_C$ and $S_M$.  Again, we use VGG3.2
  %layer as an example.
%
  %We then tighten the bound, by considering the amount of available
  %cache of a given processor.  We show that this way, of three--stage
  %sequential computation, allows for the fastest computation.
  %Finally, we show that, on modern ConvNets, the FFT/FFT+Gauss
  %convolution have lower bounds in computation time compared to
  %Winograd.
%
  %Similarly as in the previous section, we analyze an arbitrary sized
  %Winograd convolution ($F(m^2,r^2)$), and arbitrary sizes
  %FFT/FFT+Gauss convolutions
  %($\mathcal{F}(m^2,r^2)$/$\mathcal{F}_G(m^2,r^2)$).
%
  %\subsection{Memory Requirements}
%
  %Storing all input images as 32--bit floating point numbers requires
  %$4BCx^2$ bytes, where $B$ is the batch size, $C$ is the number of
  %input channels and $x^2$ is the size of each image.  Similarly,
  %storing all output images require $4BC'y^2$ bytes, $y^2$ is the size
  %of the output images.  In the case of VGG3.2 (Row X in
  %Tbl.~\ref{table:complexities}), $x=y$, as the input images are
  %implicitly padded, and then reduced to the same size after the
  %convolutions.  Kernels require $4CC'r^2$ bytes of memory; $r^2$ is
  %the kernel size.
%
  %Each of $B \cdot C$ input images is divided into
  %$\ceil{(d-r+1)/m}^2$ tiles, where $d$ is the input image size
  %adjusted for the implicit padding ($d = x + 2p$).  In
  %Winograd--based convolution, each tile contains $(m+r-1)^2$ real
  %numbers; the memory required for storing the transformed input tiles
  %is $4BC\ceil{(d-r+1)/m}^2(m+r-1)^2$ bytes.  In FFT--based
  %convolution, tiles contain $\ceil{(m+r)/2}(m+r-1)$ complex numbers
  %(twice as many real numbers), requiring total of
  %$8BC\ceil{(d-r+1)/m}^2\ceil{(m+r)/2}(m+r-1)$ bytes.  When Gauss's
  %multiplication is used, complex numbers are represented by three
  %real numbers, requiring 1.5x more memory.
%
  %There are same number of tiles per output an image as per an input
  %image.  The memory required for the pre--transformed outputs can be
  %calculated in similar fashion (replacing $C$ with $C'$ in the
  %formulas above).
%
  %There is a single tile for each of the $CC'$ transformed kernels,
  %requiring total of $4CC'(m+r-1)^2$ bytes for Winograd,
  %$8CC'\ceil{(m+r)/2}(m+r-1)$ for FFT, and
  %$12CC'\ceil{(m+r)/2}(m+r-1)$ for FFT+Gauss.
%
  %\subsection{Compute--to--memory Ratios}
%
  %Knowing the amount of FLOPs, and the amount of memory that has to be
  %read/written, we can estimate the compute--to--memory ratio for each
  %stage.
%
  %To perform input transforms, we need to read the original images and
  %store the transformed inputs.  Similarly, to transform kernels, we
  %need to read the all kernels and store their transforms.  To perform
  %the element--wise product, we need to read all transformed images
  %and kernels, and store the transformed outputs.  Finally, the
  %perform the inverse transforms we need to read the transformed
  %output images and store the final output images.
%
  %The estimate of the compute--to--memory ratios for the four stages
  %are given in Tbl.~\ref{table:complexities} (row x-y).
%
  %This estimates assume that each location in the main memory is read
  %from/stored to exactly once.  This is a fair assumption for the
  %transformation stages, as we can read a subset of the
  %images/kernels/transformed outputs, perform the computation in
  %cache, and store the result back to main memory -- thus accessing
  %each location in main memory exactly once.
%
  %In the element--wise product stage, however, we might need to access
  %some memory locations multiple times, which reduces the
  %compute--to--memory ratio of the stage.
%
  %\subsubsection{Element--wise computation}
%
  %Element--wise product stage performs a set matrix multiplications
  %($Z = X \stimes Y$, where $Z$ and $X$ have sizes $W \stimes C$ and
  %$W \stimes C'$; $Y$ has size of $C \stimes C'$.~\cite{many}.  For
  %each tile of each image, there is a single row in matrices $Z$ and
  %$X$, thus $W = BC\ceil{(d-r+1)/m}^2$.  For all modern ConvNets this
  %value is much larger than $C$ and $C'$, rendering matrices $X$ and
  %$Z$ tall and relatively skinny.
%
  %\begin{figure}
    %\begin{center}
      %\includegraphics[width=0.48\linewidth]{fig/gemm_ratios.pdf}
      %\includegraphics[width=0.48\linewidth]{fig/cgemm_ratios.pdf}
    %\end{center}
    %\caption{}
    %\label{fig:gemm-cgemm-ratios}
  %\end{figure}
%
  %Maximizing the compute--to--memory ratio of multiplication of tall
  %and skinny matrices has been well studied~\cite{many}.  To minimize
  %the number of memory accesses, the matrix $Y$ is kept in cache; few
  %row of $X$ are then fetched from memory to compute the same number
  %of rows of $Z$.  To compute a single row of $Z$, a row of $X$ has to
  %be fetched from main memory, the product with $Y$ is computed in
  %cache, and the result is stored back to main memory.  With $Y$ in
  %cache, the compute--to--memory ratio can be estimated to
  %$CC'/2(C+C')$ for real valued matrices, and to $CC'/(C+C')$ for
  %complex valued matrices.  This requires a cache capable of storing
  %the matrix $Y$ and single rows of $X$ and $Z$ - total of $C + C' +
  %CC'$ floating point numbers.
%
  %When that is not possible, cache blocking strategies are employed.
  %The matrix multiplication is decomposed into many multiplications
  %with smaller matrices.  The matrix $Y$ is subdivided into smaller
  %matrices $y_i$ of size $c \stimes c'$, where $c \le C$ and $c' \le
  %C'$; with $C$ and $C'$ being divisible by $c$ and $c'$ respectively.
%
  %When $c < C$, each row of $Z$ is computed as a sum of two or more
  %matrix multiplications - the results of matrix multiplications in
  %the decomposition have to be accumulated, this requiring extra
  %memory access (to fetch previously computed values to accumulate
  %to).
%
  %For given decomposition with $c \le C$ and $c' \le C'$, the
  %compute--to--memory ratio of each matrix multiplication (and thus
  %the overall computation) is: {\small
  %\begin{equation}
    %\frac{\beta cc'}{2(c + \alpha c')}
  %\end{equation}
  %} And requires $4 \beta(cc' + c + \alpha c')$ bytes of cache.  Here,
  %$\beta$ is $1$ for real valued matrices, and $2$ for complex ones;
  %$\alpha$ equals to $1$ when $c = C$, and $2$ when $c < C$.
%
  %For a given cache size, $C$ and $C'$, we can find optimal
  %decomposition ($c$ and $c'$) such that the compute--to--memory ratio
  %is maximized; we obtain this by exhaustive search, and show the
  %results on Fig.~\ref{fig:gemm-cgemm-ratios}.
%
  %This gives us the maximal possible memory--to--compute ratio, for
  %the element--wise stage as a function of cache size.
  %Winograd--based convolution uses real valued matrix multiplication,
  %and FFT uses complex valued ones.  Gauss's complex number
  %multiplication is performed by $3$ independent multiplications of
  %real valued matrices; thus, the FFT+Gauss approach has the same
  %limit on the memory--to--compute ratio as Winograd (Row Z on
  %Tbl.~\ref{table:complexities}.
%
  %\subsection{Minimal Compute Times}
%
  %For a given processor (given $S_C$, $S_M$) we can compute the
  %estimated time required for performing computation of each of the
  %stages using the Eqn.~\ref{eqn:times}.
%
  %The compute--to--memory ratios of the transformation stages are much
  %lower than the compute--to--memory ratios of modern processors.
  %From Tbl.~\ref{table:complexities} we see that for all methods and
  %all transforms, the ratio is below $2.3$, while modern processors
  %have much larger ratios.  This ratio depends on the transform size,
  %for both Winograd and FFT.  We have computed this ratio for
  %transform sizes $F(m^2,r^2)$, $(2 \le m \le 8, 2 \le r \le 8)$ for
  %Winograd, and $\mathcal{F}(m^2,r^2)$, $(2 \le m \le 32, 2 \le r \le
  %8)$ for FFT and FFT+Gauss.  The compute--to--memory ratio is always
  %below $4$.
%
  %This means that on modern processors, the transform stages, will
  %always be memory--bound.  It also has an interesting implication,
  %that using very obscure FFT transform sizes, such as large prime
  %numbers, could be very efficient.  This is in direct contrast to all
  %FFT--based approaches, which use only power of two transform sizes,
  %for which faster algorithms are known~\cite{many}.
  %\aleks{STRONGER!}
%
  %The memory--to--compute ratio of the element--wise product stage
  %might be limited by the processor it is running on.
%
  %As an example, we estimate the time required for each approach on
  %two processors.  KNL ($S_C = 4.5$ TFLOPS, $S_M = 400$ GB/s, $256$ KB
  %of L2 cache) and SKX ($S_C = 2.1$ TFLOPS, $S_M = 96$ GB/s, $512$ KB
  %of L2 cache).  The compute--to--memory ratios of KNL was $11.3$ and
  %of SKX $22$.
%
  %\subsection{Speed of FFT vs Winograd}
%
  %\begin{figure*}
    %\begin{center}
      %\includegraphics[width=0.47\linewidth]{fig/layers3b.pdf}
      %\includegraphics[width=0.47\linewidth]{fig/layers4b.pdf}
    %\end{center}
    %\caption{Theoretical Speedup of FFT vs Winograd.}
    %\label{fig:layers1-speedup}
  %\end{figure*}
%
  %Total time required is the sum over stages.
  %{\small
    %\label{eqn:times}
  %\begin{equation}
    %\sum_i \frac{N^i_M}{S_C}\min\{N^i_R,S_R\}
  %\end{equation}
  %} Thus, the relative speeds of any two approaches depend solely on
  %$S_R$, as $S_C$ cancels out.  For a given layer, the relative speed
  %of Winograd and FFT approaches, for different transform sizes, will
  %depend solely on $S_R$ of a given processor, from
  %Eqn.~\ref{eqn:times}.
%
  %We consider the convolutional layers of three popular ConvNets -
  %VGG, AlexNet and OverFeat.  To estimate the fastest computation
  %time, using Winograd--based convolution $F(m^2,r^2)$, we perform the
  %same analysis as shown in Tbl.~\ref{table:complexities}, as a
  %function of $S_R$.
%
  %The value
  %of $r$ is fixed to the size of the kernel of the particular layer,
  %and we vary the value of $m$ between 2 and 6, as larger values are
  %numerically unstable.  Similarly, for both $\mathcal{F}(m^2,r^2)$
  %and $\mathcal{F}_G(m^2,r^2)$, we vary $m$ between 2 and 32.  On
  %Fig.~\ref{fig:layers1-speedup} we plot the ratio between the
  %estimated computation time of the fastest FFT--based approach and
  %fastest Winograd--based approach for the same layer (solid lines),
  %as well as the ratio between the fastest FFT+Gauss and fastest
  %Winograd--based approach (dotted lines).
%
%\remove{
%
  %\subsection{Fused vs Non--Fused Computation}
%
  %Our estimate of the number of FLOPs required assumed ``non--fused''
  %computation.  That is, the computation is performed in three
  %separated stages, where first the inputs and kernels are
  %transformed, and stored back to memory.  After that the
  %element--wise computation is performed, storing the results, again,
  %back to memory.  Finally, the output transforms are performed.  As
  %the results in Tbl.~\ref{table:complexity} suggest, the computation
  %is usually dominated by the element--wise computation stage.
%
  %To avoid the memory overhead, a ``fused'' computation can be
  %performed, as originally suggested and implemented by Lavin et
  %al.~\cite{lavin2016fast}.  A subset of the input images and kernels
  %are transformed, then element--wise computation and output
  %transforms are performed, while keeping all the data in either the
  %cache or the register file.
%
  %Counterintuitively, despite the memory overhead, on modern
  %processors, the non--fused approach can better utilize the hardware.
  %This is due to the relatively high compute to memory ratio, and
  %relatively low cache and register file sizes, as shown in the
  %analysis below.
%
  %Semi--fused approaches are also possible.  As in the fused case, a
  %subset if the problem is computed at the time, but allowing for
  %temporary results to be stored in main memory.  This approach can
  %reduce the memory size required for temporary data, but has the same
  %number of memory accesses as the non--fused approach.
%
  %One of the main motivations for using fused approach is to reduce
  %the size of the scratch memory required~\cite{lavin2016fast}, due to
  %the limited size of available GPU memory.  However, modern GPUs have
  %relatively large amount of on--board RAM.  Modern ConvNets are very
  %deep, and the non--fused approach requires as much memory as an
  %additional layer.  In practice, the non--fused approach uses half a
  %dozen percents of the available memory, which can be further reduced
  %by using semi--fused approach.
%
  %\subsubsection{Cache required for fused computation}
%
  %In fused computation, $k \le K$ input tiles from each of the $c \le
  %C$ input channels are transformed to produce $c' \le C'$ output
  %tiles.
%
%\zhen{N means T?}
  %For the case of Winograd transform, the total amount of computation
  %is then $O_{in}(kc) + O_{ker}(cc') + O_{out}(kc') + 2Nkcc'$.  Here
  %$O_{in}(kc)$ is the number of floating operations required for
  %transforming the input tiles, $O_{ker}(cc')$ for transforming
  %kernels, and $O_{out}(kc')$ for transforming the outputs.  The
  %$2Tkcc'$ is the number of operations required for the element--wise
  %multiplications, where $T$ is the tile size (number of elements in a
  %single tile).
%
  %We need to fetch the $kc$ input tiles and $cc'$ kernels from memory,
  %as well as store the resulting $kc'$ output tiles back.
  %Additionally, when $c < C$, additional $kc'$ output tiles have to be
  %fetched from memory.  Additionally, three ways of cache/register
  %blocking can be performed.  Any of the three values: input
  %transforms, kernel transforms or output transforms can be kept in
  %cache and reused.
%
  %For the Winograd--based convolution using $F(m \stimes m,n \stimes
  %n)$, the compute to memory ratio is
  %{\small
  %\begin{equation}
    %\frac{O_{trans} + 2t^2kcc'} {\min\{n^2cc' + \alpha m^2kc',t^2kc +
      %\alpha m^2kc',t^2kc + n^2cc''\}}
  %\end{equation}
  %} Where $t = m + n - 1$ (input image tile size), and $\alpha$ is
  %either 1 or 2 (depending on whether $c < C$).  At the same time, in
  %order to perform in--cache computation, we need to be able to fit
  %$kc$ transformed input tiles, $cc'$ transformed kernel tiles, and
  %$kc'$ output tiles inside the cache and register file -- total of $K
  %= t^2kc + t^2cc' + t^2kc'$ floating point numbers.
%
  %For a given compute to memory ratio, we can find optimal $k$, $c$
  %and $c'$ such that $K$ is minimized.  Such value of $K$ represents
  %the minimal amount of cache and register file required in order to
  %achieve that ratio.
%
  %For a Winograd transform $F(m \stimes m,n \stimes n)$, the exact value
  %of $O_{trans}$ can be computed using the code generator of~\cite{}.
  %We can than solve the optimization problem -- find $k, c$ and $c'$
  %such that the required cache/register memory $K$ is minimized, and
  %the compute to memory ratio is larger than a given one.  Only
  %integral values for $k, c$ and $c'$ are allowed.
%
  %\begin{figure}
    %\begin{center}
      %\includegraphics[width=0.48\linewidth]{fig/fused_ratios_23.pdf}
      %\includegraphics[width=0.48\linewidth]{fig/fused_ratios_43.pdf}
    %\end{center}
    %\caption{Lower bound on cache/register file size required in order
      %to saturate processors with different compute to memory ratios
      %for F(2x2,3x3) (left) and F(4x4,3x3) (right).}
    %\label{fig:cache-required}
  %\end{figure}
%
  %On Fig.~\ref{fig:cache-required} we show the lower bound on the
  %cache/register file required for winograd transforms of F(2x2,3x3)
  %and F(4x4,3x3).  This is very conservative memory bound because: (1)
  %depending on the processor, only certain values for $k$, $c$ and
  %$c'$ might be allowed in order to fully utilize the processor
  %(depending on the vector register size); (2) we assume that we can
  %perfectly fit the data in the cache/register file; and (3) in order
  %to hide latency, the cache size and values for $k$, $c$ and $c'$
  %might be further restricted.  On the GPU, one needs to run multiple
  %blocks per SM in order to hide latency, thus lowering cache
  %available per block.  Similarly, the values of $k$ need to be larger
  %than the latency of the FMA instructions for the CPU. \aleks{Maybe
    %too much?}.
%
  %We examine the possibility of implementing the fused approach on two
  %CPUs and two GPUs.  Titan X and Titan X Pascal have 24 and 28 SMs
  %respectively.  Each SM has 64K of memory that can be used as L1
  %cache or register file.  Additionally, both GPUs have 3MB of shared
  %L2 cache.  This gives total of 192KB/173KB cache memory per SM for
  %the two GPUs.  The KNL CPU has 256KB and the SKX has 512KB L2 cache
  %per core.
%
%\zhen{I think, we may delete this paragraph. I mean, if we have more space, we can keep it to further support our analysis.}
  %On the GPU, it is only theoretically possible to fully utilize the
  %Titan X for F(2,3).  This can be achieved with an algorithm
  %suggested by Lavin et al.~\cite{lavin2016fast}, which was indeed
  %tested on the Titan X GPU.  Lavin et al. also suggests that the
  %fused approach of Winograd F(4,3) is not possible.  On newer GPUs
  %with higher compute to memory ratio (such as Titan X Pascal) even
  %F(2,3) can not be efficiently implemented.  CuDNN, starting from
  %version 6, provides both fused and non--fused implementation of the
  %Winograd convolution, which confirms our theoretical findings -- the
  %non--fused is much faster, but requires less memory, on both Titan X
  %and Titan X Pascal.
%
  %Our data suggests that F(2,3) is theoretically possible on both KNL
  %and SKX, while F(4,3) is not.  In practice, implementing fused
  %F(2,3) is both difficult (\aleks{explain... cache associativity})
  %and not practical, as F(4,3) requires much less computation, and
  %memory is not an issue on the CPU.
%
  %Similar analysis can be performed for larger tile sizes for both the
  %Winograd and FFT--based convolutions.  However, as the cache
  %required strongly depends on the tile size, and for the FFT--based
  %convolutions we expect to use much larger tiles, we can conclude
  %that fused (and efficient) FFT--based convolution is not viable.
%}

